Enhancing Virtual Ontology Based Access over Tabular Data with Morph-CSV

Ontology-Based Data Access (OBDA) has traditionally focused on providing a unified view of heterogeneous datasets, either by materializing integrated data into RDF or by performing on-the fly querying via SPARQL query translation. In the specific case of tabular datasets represented as several CSV or Excel files, query translation approaches have been applied by considering each source as a single table that can be loaded into a relational database management system (RDBMS). Nevertheless, constraints over these tables are not represented; thus, neither consistency among attributes nor indexes over tables are enforced. As a consequence, efficiency of the SPARQL-to-SQL translation process may be affected, as well as the completeness of the answers produced during the evaluation of the generated SQL query. Our work is focused on applying implicit constraints on the OBDA query translation process over tabular data. We propose Morph-CSV, a framework for querying tabular data that exploits information from typical OBDA inputs (e.g., mappings, queries) to enforce constraints that can be used together with any SPARQL-to-SQL OBDA engine. Morph-CSV relies on both a constraint component and a set of constraint operators. For a given set of constraints, the operators are applied to each type of constraint with the aim of enhancing query completeness and performance. We evaluate Morph-CSV in several domains: e-commerce with the BSBM benchmark; transportation with a benchmark using the GTFS dataset from the Madrid subway; and biology with a use case extracted from the Bio2RDF project. We compare and report the performance of two SPARQL-to-SQL OBDA engines, without and with the incorporation of MorphCSV. The observed results suggest that Morph-CSV is able to speed up the total query execution time by up to two orders of magnitude, while it is able to produce all the query answers.

==> algorithm/algorithm.tex <==
\begin{algorithm}[H]
\SetAlgoLined
\KwResult{OBDA instance PI}
 initialization\;
 \forall tp \in Q
 \While{While condition}{
  instructions\;
  \eIf{condition}{
   instructions1\;
   instructions2\;
   }{
   instructions3\;
  }
 }
 \caption{Morph-CSV algorithm}
\end{algorithm}

==> aux.tex <==
\begin{table*}[t]
\centering
\caption{Query evaluation performance (time in seconds) over multiple sizes of a GTFS dataset (the number indicates the scale factor: 1, 10, 100 and 100), The absence of a value means that the OBDA engine does not support the features of the SPARQL query. Execution time is a lower-is-better metric; best results are highlighted in \textbf{bold}.}
\label{tab:gtfs-results}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c}
\hline
\multicolumn{1}{c|}{\textbf{Engines/Queries}} & \textbf{Q1} & \textbf{Q2} & \textbf{Q4} & \textbf{Q6} & \textbf{Q7} & \textbf{Q9} & \textbf{Q12} & \textbf{Q13} & \textbf{Q17} & \textbf{\begin{tabular}[c]{@{}c@{}}Geometric\\  Mean\end{tabular}} \\ \hline
\multicolumn{11}{c}{\textbf{GTFS-1}} \\ \hline
\textbf{Morph-RDB} & \textbf{6,94} & \textbf{3,04} & \textbf{2,78} & \textbf{2,78} & \textit{timeOut} & \textit{timeOut} & 6,23 & \textbf{3,97} & \textbf{3,14} & 20,56\\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Morph-CSV \&\\ Morph-RDB\end{tabular}} & 8,18 & 4,22 & 4,01 & 3,91 & \textbf{4,31} & \textbf{24,15} & \textbf{4,22} & 4,39 & 4,42 & \textbf{5,50} \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Ontop\end{tabular}} & 9,93 & 6,60 & - & - & - & - & - & 6,62 & 6,56 & 7,30 \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Morph-CSV \&\\ Ontop\end{tabular}} & 11,54 & 8,36 & - & - & - & - & - & 8,25 & 8,32 & 9,02 \\ \hline
\multicolumn{11}{c}{\textbf{GTFS-10}} \\ \hline
\textbf{Morph-RDB} & 25,90 & 6,06 & 5,20 & 4,89 & \textit{timeOut} & \textit{timeOut} & \textit{timeOut} & 38,15 & 38,90 & 109,21 \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Morph-CSV \&\\ Morph-RDB\end{tabular}} & \textbf{23,99} & \textbf{5,01} & \textbf{4,20} & \textbf{3,84} & \textbf{4,87} & \textbf{93,72} & \textbf{9,58} & \textbf{4,92} & \textbf{5,50} & \textbf{8,49} \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Ontop\end{tabular}} & 37,97 & 19,48 & - & - & - & - & - & 19,21 &	19,54 & 22,95 \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Morph-CSV \&\\ Ontop\end{tabular}} & 77,73 & 8,80 & - & - & - & - & - & 8,50 & 8,62 & 14,96 \\ \hline
\multicolumn{11}{c}{\textbf{GTFS-100}} \\ \hline
\textbf{Morph-RDB} & \textit{timeOut} & 43,59 & 38,52 & 38,43 & \textit{timeOut} & \textit{timeOut} & \textit{timeOut} & \textit{timeOut} & \textit{timeOut} & 1276,35 \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Morph-CSV \&\\ Morph-RDB\end{tabular}} & 205,99 & \textbf{9,88} & \textbf{4,90} & \textbf{3,99} & \textbf{9,07} & \textit{timeOut} & \textbf{11,53} & \textbf{8,54} & \textbf{11,88} & \textbf{11,97} \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Ontop\end{tabular}} & 1513,72 & 45,21 & - & - & - & - & - & 43,14	& 45,54 & 107,68 \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Morph-CSV \&\\ Ontop\end{tabular}} & \textbf{127,06} & 14,26 & - & - & - & - & - & 10,67 & 12,75 & 22,28 \\ \hline
\multicolumn{11}{c}{\textbf{GTFS-1000}} \\ \hline
\textbf{Morph-RDB} & \textit{timeOut} & \textit{timeOut} & \textit{timeOut} & \textit{timeOut} & \textit{timeOut} & \textit{timeOut} & \textit{timeOut} & \textit{timeOut} & \textit{timeOut} & \textit{timeOut} \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Morph-CSV \&\\ Morph-RDB\end{tabular}} & \textit{timeOut} & \textbf{93,86} & \textbf{7,01} & \textbf{4,24} & \textbf{66,35} & \textit{timeOut} & \textbf{71,43} & \textbf{44,29} & \textbf{68,84} & \textbf{32,74} \\ \hline
\textbf{Ontop} & \textit{timeOut} & \textit{timeOut} & - & - & - & - & - & \textit{timeOut} & \textit{timeOut} & \textit{timeOut} \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Morph-CSV \&\\ Ontop\end{tabular}} & \textit{timeOut} & \textit{timeOut} & - & - & - & - & - & 274,93 & 1252,40 & 2055,46 \\ \hline
\end{tabular}%
%}
\end{table*}


\noindent\textbf{Step 1: Source Selection.} Before starting the application of constraints, Morph-CSV takes as input the SPARQL query, the set of mapping rules and the tabular dataset, and %performs the function $select(Q,M_{tabular},S_{lw})$. The function 
uses the information encoded in the query and the rules of the mapping to only select the files and columns from $S_{lw}$ that are required to answer the query. After that, Morph-CSV also removes the irrelevant rules from the mapping document. The output of this step is a new OBDAT instance $IT^{'}$ where the number of results of $evalt(Q,IT)$ is the same as $evalt(Q,IT^{'})$. This function tackles the \textit{Selection} challenge identified in Section~\ref{sec:challenges}. Note that the following steps are executed over the selected data sources and columns.

\noindent\textbf{Step 2: Data Normalization} There are two functions for performing  data normalization. The first one is the treatment of multi-values in a column. In this case, Morph-CSV performs the function $split(A_{i},S_{j},sep)$ where $A_{i}$ is the multi-valued column of  source $S_{j}$ and $sep$ is the character defined in the metadata that divides the values (e.g., $split$(date,stops,-). The application of this function is known as the normalization step for 2NF~\cite{codd1979extending}. 

The second function is the treatment of multiple entities in the same source. Morph-CSV takes the mapping rules and the lightweight schema and executes the function $cut(\mathcal{M}_{tabular},\mathcal{S}_{lw})$. This function analyzes the mapping rules $\mathcal{M}_{tabular}$ and performs a   3NF~\cite{codd1979extending} normalization step over $S_{lw}$, when there are two sets of mapping rules that have the same source and the intersection of their references is empty. 
Additionally, both functions  rewrite the mapping rules according to the changes performed over the lightweight tabular schema. These functions tackle the \textit{Normalization} challenge and their output is a new OBDAT instance $IT^{'}$.

\noindent\textbf{Step 3: Data preparation} In this step, Morph-CSV addresses the challenge of \textit{Heterogeneity} and performs two different functions: $sub$ and $create$. The first one is defined as $sub(exp(A_{i}),S_{j},val)$ where $exp(A_{i})$ is a boolean function over column $A_{i}$ of source $S_{j}$ that when true, the value of $A_{i}$ is substituted by $val$. For example, the GTFS spec in the exception\_type column in the calendar\_dates.csv file, the value 2 means false. To prepare the data to be queried, Morph-CSV extracts that information from the tabular metadata and performs the function $sub(exception\_type=2,calendar\_dates.csv,false)$. There are multiple substitution functions that Morph-CSV executes such as default values, null values and date formats. The second function creates a new column in a specific source $S_{j}$. It is defined as $create(c(A_{n},\ldots,A_{m}),S_{j})$, where $c(A_{n},\ldots,A_{m})$ means the application of a set of transformation functions over the columns $A_{n},\ldots,A_{m}$ from  source $S_{j}$. This function is used when ad-hoc transformations functions are needed and it is usually defined inside the mapping rules~\cite{junior2016funul,de2017declarative}. For example, to give the same structure to stop names in GTFS, the function is defined as $create(lower(replace(name,$\textbackslash$ s+,\_)),stops.csv)$. Additionally, at the end of this step, Morph-CSV removes all the duplicates generated over the raw data applying the ideas describe in~\cite{jozashoori2019mapsdi}, which have an important impact in the behavior of the engines. The output of both functions is a new OBDAT instance $IT^{'}$.

\noindent\textbf{Step 4: Schema Creation and Load.} The final step before translating and executing the query is to create an SQL schema applying a set of constraints and a function to load the tabular data sources. The constraints that Morph-CSV incorporates in this step are $primaryKey(A_{i},S_{j})$, $foreignKey(A_{i},S_{j})$, $index(A_{i},S_{j})$ and $dataType(A_{i},S_{j},type)$, that are typical constraints applied in SQL-based systems. However, Morph-CSV exploits the information encoded in the query to apply a set of heuristics in this process with the aim of improving query execution. First, the integrity constraints ($primaryKey$,$foreignKey$) are only applied in the case that the query performs a join among the references of these constraints. Additionally, the application of the $index$ constraints is based on the selectivity of a column $A$ and the query filters, i.e., the engine decides on-the-fly to create an index based on these inputs. Finally, the data is loaded in a RDB following the newly created schema. This step tackles the problem of \textit{Lightweight Schema} and its output is an OBDA instance $I^{'}$ that can be the input to any SPARQL-to-SQL OBDA engine. 




%\begin{table*}[t]
%\centering
%\caption{Query completeness over multiple sizes of a GTFS dataset (the number indicates the scale factor: 1, 10, 100 and 100). The absence of a value means that the OBDA engine does not support the features of the SPARQL query. }
%\label{tab:gtfs-complete}
%\resizebox{\textwidth}{!}{%
%\begin{tabular}{l|c|c|c|c|c|c|c|c|c}
%\hline
%\multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Engines/\\ Queries\end{tabular}}} & \textbf{Q1} & \textbf{Q2} & \textbf{Q4} & \textbf{Q6} & \textbf{Q7} & \textbf{Q9} & \textbf{Q12} & \textbf{Q13} & \textbf{Q17} \\ \hline
%\multicolumn{10}{c}{\textbf{GTFS-1}} \\ \hline
%\textbf{Virtuoso} & 58540 & 765 & 13 & 1 & 2 & 151439 & 6 & 734 & 855 \\ \hline
%\textbf{Morph-RDB} & 58540 & 765 & 13 & 1 & \textit{timeOut} & \textit{timeOut} & 6 & 734 & 855 \\ \hline
%\textbf{\begin{tabular}[c]{@{}l@{}}Morph-CSV \&\\ Morph-RDB\end{tabular}} & 58540 & 765 & 13 & 1 & 2 & 151439 & 6 & 734 & 855 \\ \hline
%\textbf{\begin{tabular}[c]{@{}l@{}}Ontop\end{tabular}} & 58540 & 765 & - & - & - & - & - & 734 & 855 \\ \hline
%\textbf{\begin{tabular}[c]{@{}l@{}}Morph-CSV \&\\ Ontop\end{tabular}} & 58540 & 765 & - & - & - & - & - & 734 & 855 \\ \hline
%\multicolumn{10}{c}{\textbf{GTFS-10}} \\ \hline
%\textbf{Virtuoso} & 353660 & 6312 & 130 & 1 & 67 & 718317 & 130 & 2650 & 8550 \\ \hline
%\textbf{Morph-RDB} & 353660 & 6312 & 130 & 1 & \textit{timeOut} & \textit{timeOut} & \textit{timeOut} & 2650 & 8550 \\ \hline
%\textbf{\begin{tabular}[c]{@{}l@{}}Morph-CSV \&\\ Morph-RDB\end{tabular}} & 353660 & 6312 & 130 & 1 & 67 & 718317 & 130 & 2650 & 8550 \\ \hline
%\textbf{\begin{tabular}[c]{@{}l@{}}Ontop\end{tabular}} & 353660 & 6312 & - & - & - & - & - & 2650 & 8550 \\ \hline
%\textbf{\begin{tabular}[c]{@{}l@{}}Morph-CSV \&\\ Ontop\end{tabular}} & 353660 & 6312 & - & - & - & - & - & 2650 & 8550 \\ \hline
%\multicolumn{10}{c}{\textbf{GTFS-100}} \\ \hline
%\textbf{Virtuoso} & 3536600 & 63100 & 1300 & 1 & 67 & 7183874 & 1300 & 26500 & 85500 \\ \hline
%\textbf{Morph-RDB} & \textit{timeOut} & 63100 & 1300 & 1 & \textit{timeOut} & \textit{timeOut} & \textit{timeOut} & \textit{timeOut} & \textit{timeOut} \\ \hline
%\textbf{\begin{tabular}[c]{@{}l@{}}Morph-CSV \&\\ Morph-RDB\end{tabular}} & 3536600 & 63100 & 1300 & 1 & 67 & timeOut & 1300 & 26500 & 85500 \\ \hline
%\textbf{\begin{tabular}[c]{@{}l@{}}Ontop\end{tabular}} & 3536600 & 63100 & - & - & - & - & - & 26500 & 85500 \\ \hline
%\textbf{\begin{tabular}[c]{@{}l@{}}Morph-CSV \&\\ Ontop\end{tabular}} & 3536600 & 63100 & - & - & - & - & - & 26500 & 85500 \\ \hline
%\multicolumn{10}{c}{\textbf{GTFS-1000}} \\ \hline
%\textbf{Virtuoso} & 35366000 & 1261368 & 13000 & 1 & 69 & 19077083 & 13000 & 420666 & 855000 \\ \hline
%\textbf{Morph-RDB} & \textit{timeOut} & \textit{timeOut} & \textit{timeOut} & %\textit{timeOut} & \textit{timeOut} & \textit{timeOut} & \textit{timeOut} & \textit{timeOut} & \textit{timeOut} \\ \hline
%\textbf{\begin{tabular}[c]{@{}l@{}}Morph-CSV \&\\ Morph-RDB\end{tabular}} & \textit{timeOut} & 1261368 & 13000 & 1 & 69 & - & 13000 & 420666 & 855000 \\ \hline
%\textbf{\begin{tabular}[c]{@{}l@{}}Ontop\end{tabular}} & \textit{timeOut} & \textit{timeOut} & - & - & - & - & - & \textit{timeOut} & \textit{timeOut} \\ \hline
%\textbf{\begin{tabular}[c]{@{}l@{}}Morph-CSV \&\\ Ontop\end{tabular}} & \textit{timeOut} & \textit{timeOut} & - & - & - & - & - & 420666 & 855000 \\ \hline
%\end{tabular}%
%}
%\end{table*}


\begin{table*}[t]
\centering
\caption{Summary of constraints and corresponding functions applied by Morph-CSV. The proposed steps and their relation with the input, the output performed by each function, and the addressed challenge.}
\label{tab:summary}
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{l|l|l|l|l|l}
\hline
\multicolumn{1}{c|}{\textbf{Step}} & \multicolumn{1}{c|}{\textbf{Constraint}} & \multicolumn{1}{c|}{\textbf{Function}} & \multicolumn{1}{c|}{\textbf{Input}} & \multicolumn{1}{c|}{\textbf{Output}} & \multicolumn{1}{c}{\textbf{Challenge}} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Data\\ Normalization\end{tabular}} & 2NF & split & \begin{tabular}[c]{@{}l@{}}Column, Source, \\ Separator\end{tabular} & \begin{tabular}[c]{@{}l@{}}Schema, Data,\\ Mappings\end{tabular} & \multicolumn{1}{c}{\multirow{2}{*}{Normalization}} \\ \cline{2-5}
 & 3NF & cut & Mappings, Schema & Schema & \multicolumn{1}{c}{} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Data\\ Preparation\end{tabular}} & \multirow{2}{*}{Standardization} & sub & \begin{tabular}[c]{@{}l@{}}Expression, Column,\\ Source, Value\end{tabular} & Data & \multirow{2}{*}{Heterogeneity} \\ \cline{3-5}
 &  & create & \begin{tabular}[c]{@{}l@{}}Expression, Columns,\\ Source\end{tabular} & \begin{tabular}[c]{@{}l@{}}Data\\ Query\end{tabular} &  \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Schema\\ Creation and\\ Load\end{tabular}} & Primary Key & primaryKey & \begin{tabular}[c]{@{}l@{}}Column, Source,\\ Query\end{tabular} & Schema & \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Lightweight \\ Schema\end{tabular}} \\ \cline{2-5}
 & Foreign Key & foreignKey & \begin{tabular}[c]{@{}l@{}}Column, Source,\\ Query\end{tabular} & Schema &  \\ \cline{2-5}
 & DataType & datatype & \begin{tabular}[c]{@{}l@{}}Column, Source,\\ Query\end{tabular} & Schema &  \\  \hline
\end{tabular}%
}
\end{table*}
